HOT-VAE: Learning High-Order Label Correlation for Multi-Label Classification via Attention-Based Variational Autoencoders

Understanding how environmental characteristics affect bio-diversity patterns, from individual species to communities of species, is critical for mitigating effects of global change. A central goal for conservation planning and monitoring is the ability to accurately predict the occurrence of species communities and how these communities change over space and time. This in turn leads to a challenging and long-standing problem in the field of computer science - how to perform ac-curate multi-label classification with hundreds of labels? The key challenge of this problem is its exponential-sized output space with regards to the number of labels to be predicted.Therefore, it is essential to facilitate the learning process by exploiting correlations (or dependency) among labels. Previous methods mostly focus on modelling the correlation on label pairs; however, complex relations between real-world objects often go beyond second order. In this paper, we pro-pose a novel framework for multi-label classification, High-order Tie-in Variational Autoencoder (HOT-VAE), which per-forms adaptive high-order label correlation learning. We experimentally verify that our model outperforms the existing state-of-the-art approaches on a bird distribution dataset on both conventional F1 scores and a variety of ecological metrics. To show our method is general, we also perform empirical analysis on seven other public real-world datasets in several application domains, and Hot-VAE exhibits superior performance to previous methods.

==> hot-vae arxiv/abstract.tex <==
\begin{abstract}
    Understanding how environmental characteristics affect biodiversity patterns, from individual species to communities of species, is critical for mitigating effects of global change.
    A central goal for conservation planning and monitoring is the ability to accurately predict the occurrence of species communities and how these communities change over space and time.
    %An urgent need in computational sustainability is to protect biodiversity.
    %In order to prevent hundreds of species from going extinct, it is of great importance to have a better understanding of joint species distributions at different sites, which involves predicting the presence and absence of species and modelling species correlation given different environmental features.
    This in turn leads to a challenging and long-standing problem in the field of computer science - how to perform accurate multi-label classification with hundreds of labels?
    The key challenge of this problem is its exponential-sized output space with regards to the number of labels to be predicted.
    Therefore, it is essential to facilitate the learning process by exploiting correlations (or dependency) among labels.
    Previous methods mostly focus on modelling the correlation on label pairs; however, complex relations between real-world objects often go beyond second order.
    In this paper, we propose a novel framework for multi-label classification, High-order Tie-in Variational Autoencoder (HOT-VAE), which performs adaptive high-order label correlation learning.
    %Our model builds a two-branch variational autoencoder on multiple attention-based neural message passing modules.
    We experimentally verify that our model outperforms the existing state-of-the-art approaches on a bird distribution dataset on both conventional F1 scores and a variety of ecological metrics.
    To show our method is general, we also perform empirical analysis on seven other public real-world datasets in several application domains, and Hot-VAE exhibits superior performance to previous methods.
    %Ablation studies show there are a number of tradeoffs on hyper-parameter selections to better predict frequent labels or to better predict rare labels.
\end{abstract}

==> hot-vae arxiv/background.tex <==
\section{Background}
%\subsection{Notations}
Let $\mathcal D$ denote the dataset $\{(\bm{x}_i,\bm{y}_i)\}_{i=1}^N$, where $\bm{x}_i \in \mathbb R^S$ is an input and $\bm{y}_i \in \{0,1\}^L$ is an output associated with sample $i$.
Input $\bm{x}_i$ can alternatively be an ordered set of $S$ elements, and output $\bm{y}_i$ has $L$ binary labels with 1 indicating the presence and 0 indicating the absence of a label.

%In some of the text-related datasets, we use a learned embedded vector $\textbf{z}_i \in \mathbb R^d$ to represent input features $\textbf{x}_i$, where $d$ is the dimension of the embedding.
%Similarly, an embedded vector $\textbf{u}_j^{t=0}$ first represents the $j$th target, and $\textbf{u}_j^t$ where $t \geq 1$ denotes the intermediate hidden state of label $j$ after $t$ updates.

\subsection{Aligned Variational Autoencoders}
A variational autoencoder (VAE) is a generative model which consists of an encoder, a decoder, and a loss function.
The encoder, denoted by $q_\theta(\bm{z}_i|\bm{x_i})$, is a neural network that maps features of samples $\bm{x_i}$ into hidden representations $\bm{z}$, which have a much lower dimensionality than that of $\bm{x_i}$.
$\bm{z}_i$ represents a multivariate Gaussian probability density, and by sampling from this distribution we obtain noisy values of $\bm{z}_i$.
The decoder, denoted by $p_\phi(\bm{x_i}|\bm{z}_i)$, is another neural network that reconstructs $\bm{z}$ to $\bm{x_i}$.
The loss function to be minimized is $\mathbb E_{\bm{z}\sim q_\phi}[\log p_\theta(\bm{x_i}|\bm{z})]-\mathcal K [q_\phi(\bm{z}|\bm{x_i})||P(\bm{z})]$, where
$\mathcal K$ is the Kullback–Leibler (KL) divergence, and
$P(\bm{z})$ is the prior which is a standard multivariate normal distribution.
The first term encourages the reconstruction of $\bm{x_i}$, and the second term penalizes the KL divergence between the approximated distribution $q_\theta(\bm{z}|\bm{x_i})$ and the prior $P(\bm{z})$ which imposes structure on the latent space.

VAE can be used for the task of classification if the decoder is to predict target $y_i$ instead of reconstructing feature $x_i$. Therefore, we rewrite the decoder and loss function as $p_\phi(\bm{y_i}|\bm{z_x})$ and $\mathbb E_{\bm{z_x}\sim q_\phi}[\log p_\theta(\bm{y_i}|\bm{z_x})]-\mathcal K [q_\phi(\bm{z_x}|\bm{x_i})||P(\bm{z_x})]$, respectively. In this case, it is desired that the prior $P(z_x)$ imposes domain-specific structure on the latent space rather than just imposing the conventional standard multivariate normal structure. Recently, MPVAE was proposed to use another VAE to learn a latent multivariate Gaussian distribution $q_\psi(\bm{z}_{\bm{y}}|\bm{y}_i)$, and align $q_\psi(\bm{z}_{\bm{y}}|\bm{y}_i)$ and $q_\phi(\bm{z}_{\bm{x}}|\bm{x}_i)$ by penalizing their KL divergence \cite{bai2020disentangled}. The feature and label VAEs are designed to share the same decoder. Thus, the label decoder is $p_\theta(y_i|z_y)$, and the loss function can be revised as:

%Now we consider VAE-based latent embedding learning for a two-branch scheme. Given a sample $(\bm{x}_i,\bm{y}_i)$, the feature encoder maps $\bm{x}_i$ to a Gaussian subspace $\mathcal N(\mu^\psi(\bm{x}_i), \Sigma^\psi(\bm{x}_i))$ and the label encoder maps $\bm{y}_i$ to another Gaussian subspace $\mathcal N(\mu^\phi(\bm{y}_i), \Sigma^\phi(\bm{y}_i))$. To align these two subspaces, we slightly modify the original loss function for an individual sample with an additional hyper-parameter $\beta$ following MPVAE~\cite{bai2020disentangled}:
\begin{align*}
    {KL}=&\frac{1}{2}(\mathbb E_{\bm{z}_{\bm{y}} \sim q_\phi}[\log p_\theta(\bm{y}_i|\bm{z}_{\bm{y}})]+\mathbb E_{\bm{z}_{\bm{x}}\sim q_\psi}[\log p_\theta(\bm{y}_i|\bm{z}_{\bm{x}})]) \\
    &-\beta\mathcal K [q_\psi(\bm{z}_{\bm{y}}|\bm{y}_i)||q_\phi(\bm{z}_{\bm{x}}|\bm{x}_i)],
\end{align*}

where $\beta$ is a hyper-parameter to control the similarity between the two latent Gaussian distributions.

\subsection{Attention Models}

\emph{Self-attention}, sometimes called \emph{intra-attention}, is a mechanism that assigns different importance to different positions of a sequence in order to focus on more important parts.
Self-attention has been used successfully in a variety of tasks such as natural language processing (NLP) and MLC.
The Transformer and the Generative Pre-trained Transformer 3 (GPT-3) \cite{brown2020language} are two well-known attention models in NLP achieving state-of-the-art performance.
The recent Label Message Passing (LaMP)~\cite{lanchantin2019neural} can be regarded as an application of the Transformer/GPT-3 on multi-label classification.

LaMP alternates between self-attention and feed forward layers. In the $t$-th self-attention layer, each label is represented by a node $v_i^t \in \mathbb R^d$. The attention weight $a_{ij}^t$ for a node pair $(\bm{v}_i, \bm{v}_j)$ is computed as:
\begin{align}
    \label{eq:alpha}
    e^t_{ij} = a(\bm{v}^t_i,\bm{v}^t_j) = \frac{(\mathbf{W}^q\bm{v}^t_i)^{\top}
    (\mathbf{W}^u\bm{v}^t_j)}{\sqrt{\smash[b]d}} \\
    \alpha^t_{ij} = \textrm{softmax}_j(e^t_{ij}) =  \frac{\textrm{exp}(e^t_{ij})}{\sum_{k \in \mathcal{N}(i)}{\textrm{exp}(e^t_{ik})}},
\end{align}
where $a(\cdot)$ is a dot product with node-wise linear transformations $\mathbf{W}^q \in \mathbb R^{d \times d}$ on node $\bm{v}_i^t$ and $\mathbf{W}^u \in \mathbb R^{d \times d}$ on node $\bm{v}_j^t$, scaled by $\sqrt{d}$;  $e_{ij}^t$ represents the raw importance of label $j$ to label $i$ and is further normalized by a softmax function to obtain $\alpha^t_{ij}$. Then, the attention $m_i^t$ message of $v_i^t$ is generated as:
\begin{gather}
    \label{eq:m_attention}
    M_{\textrm{atn}}(\bm{v}^t_i,\bm{v}^t_j) = \alpha^t_{ij} \mathbf{W}^v \bm{v}^t_j,\\
    \bm{m}^t_i = \bm{v}^t_i + 
    \sum_{j\in \mathcal{N}(i)} M_{\textrm{atn}}(\bm{v}^t_i,\bm{v}^t_j), \label{eq:mt}
\end{gather}
where $\mathbf{W}^v \in \mathbb R^{d \times d}$ is a node-wise linear transformation.

After going through the $t$-th feed forward layer $U^t$, we obtain $v_i^{t+1}$ in the $(t+1)$-th self-attention layer as:

\begin{align}
    {\bm{v}}^{t+1}_i &= \bm{m}^t_i + U^{t}(\bm{m}^{t}_i; \bm{W}).
    \label{eq:u_attention}
\end{align}

\begin{comment}
%\paragraph{LaMP: Modelling Joint Representations by Message Passing.}
%LaMP~\cite{lanchantin2019neural} is an encoder-decoder model: the encoder operates on a feature graph where it updates feature embedding and outputs latent vectors, and the decoder operates on a label graph where it updates label embedding conditioned on the latent vectors.
LaMP uses the intra-attention (also known as self-attention) mechanism to pass messages between nodes, which enables a node to attend its neighbors differentially.
Formally, intra-attention neural message passing works as follows.
For every node, represented by $\bm{v}_i^t \in \mathbb R^d$ where $t$ indicates the time step $0\leq t \leq T$, it first computes attention weights $a_{ij}^t$ for node pairs $(\bm{v}_i, \bm{v}_j)$ using attention function $a(\cdot)$:
\begin{align}
    \label{eq:alpha}
    e^t_{ij} = a(\bm{v}^t_i,\bm{v}^t_j) = \frac{(\mathbf{W}^q\bm{v}^t_i)^{\top}
    (\mathbf{W}^u\bm{v}^t_j)}{\sqrt{\smash[b]d}} \\
    \alpha^t_{ij} = \textrm{softmax}_j(e^t_{ij}) =  \frac{\textrm{exp}(e^t_{ij})}{\sum_{k \in \mathcal{N}(i)}{\textrm{exp}(e^t_{ik})}}
\end{align}

$a(\cdot)$ is a dot product with node-wise linear $\mathbf{W}^q \in \mathbb R^{d \times d}$ on node $\bm{v}_i^t$ and $\mathbf{W}^u \in \mathbb R^{d \times d}$ on node $\bm{v}_j^t$, scaled by $\sqrt{d}$.
The result of $a(\bm{v}^t_i,\bm{v}^t_j)$ represents raw importance of label $j$ to label $i$ and is later normalized by a softmax function to obtain $\alpha^t_{ij}$.
Next, LaMP calls an attention message function $M_{atn}$ to generate a message for each neighbor of node $i$ with another transformation matrix $\mathbf{W}^v \in \mathbb R^{d \times d}$ and aggregates all messages and a residual connection on the current $\bm{v}_i^t$ to produce $\bm{m}^t_i$:

\begin{gather}
    \label{eq:m_attention}
    M_{\textrm{atn}}(\bm{v}^t_i,\bm{v}^t_j; \bm{W}) = \alpha^t_{ij} \mathbf{W}^v \bm{v}^t_j,\\
    \bm{m}^t_i = \bm{v}^t_i + 
    \sum_{j\in \mathcal{N}(i)} M_{\textrm{atn}}(\bm{v}^t_i,\bm{v}^t_j; \bm{W}). \label{eq:mt}
\end{gather}


Finally, LaMP makes an update to obtain $\bm{v}_i^{t+1}$ using a multi-layer perceptron (MLP) $U_t$:

\begin{align}
    {\bm{v}}^{t+1}_i &= \bm{m}^t_i + U_{t}(\bm{m}^{t}_i; \bm{W}).
    \label{eq:u_attention}
\end{align}

In \TODO{name}, we adopt this self-attention neural message passing module to model dependencies between labels.
\end{comment}

==> hot-vae arxiv/conclusion.tex <==
\section{Conclusion}
In this paper, we propose an attention-based HOT-VAE for multi-label classification to address the complex relations between real-world objects.
HOT-VAE learns high-order correlation between labels conditioned on features; in other words, not only can it captures relations within multiple objects, but also the relations are adaptive to any feature change.
%HOT-VAE also provides a simple and flexible way to incorporate prior knowledge by adding and removing edges in the label graphs.
Experimental results show that HOT-VAE improves over the state-of-the-art techniques.
%Further, comprehensive analysis on \emph{eBird} shows HOT-VAE makes ecologically meaningful improvements.

==> hot-vae arxiv/experiment.tex <==
\section{Experiments}
We illustrate the power of HOT-VAE on eight real-world datasets covering a variety of application domains including ecology, images, texts, etc.
We first present the main experiment, where HOT-VAE is compared to several other state-of-the-art MLC methods on all the datasets.
We evaluate their performance with conventional metrics such as F-measure and accuracy.
To verify that our model also makes a meaningful improvement in ecology, we perform analysis on 12 metrics measuring discrimination power, calibration, etc. for levels of species occurrence, species richness, and community composition~\cite{norberg2019comprehensive}.
Finally, we present ablation studies showing the benefits of having high-order label correlation and incorporating prior knowledge.

\subsection{Setup}
\paragraph{Datasets.}
The datasets we use to run experiments are: \emph{eBird}~\cite{chen2017deep}, a crowd-sourced bird presence-absence dataset collected from birders' observations; \emph{bibtex} and \emph{bookmarks}~\cite{katakis2008multilabel}, collections of text objects associated with tags; \emph{mirflickr}~\cite{huiskes08} and \emph{scene}~\cite{boutell2004learning}, collections of images with tags; \emph{reuters}~\cite{lewis2004rcv1}, natural language texts with predefined categories based on their content; \emph{sider}~\cite{kuhn2016sider}, side effects of drug molecules; and \emph{yeast}~\cite{nakai1992knowledge}, a biology database of the protein localization sites.
They are all available online~\footnote{http://mulan.sourceforge.net/datasets-mlc.html}~\footnote{https://ebird.org/home}.

These datasets vary in many aspects including the number of samples ranging from 1427 to 87856, number of labels from 6 to 208, feature dimensions from 15 to 368998.
They also cover a wide spectrum of input types: some are raw English text with words ordered sequentially, some are binary features, and the other are real-value vectors (e.g., images).
We present label statistics for each dataset in Table~\ref{tab:dataset_label_stats}, which is useful information to consider when designing models.
One can see that it is common for samples to have more than two labels.
For instance, the median number of labels per sample in $\emph{eBird}$ is 18, which suggests incorporating high-order label correlation into a model will lead to a stronger modelling capacity to learn better joint representations.

We split each dataset into a training set, a validation set, and a test set in the same way as \citet{bai2020disentangled} and \citet{lanchantin2019neural} do.

\begin{small}
\begin{table}
\scriptsize
\begin{minipage}[h]{.47\textwidth}
\centering
\scalebox{0.75}{
\begin{tabular}{c|r|r|r|r|r|r|r} 
 &\#labels  & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Mean\\ Labels\\ /Sample\end{tabular}} & \begin{tabular}[c]{@{}l@{}}Median \\ Labels\\ /Sample\end{tabular} & \begin{tabular}[c]{@{}l@{}}Max\\ Labels\\ /Sample\end{tabular} & \begin{tabular}[c]{@{}l@{}}Mean\\ Samples\\ /Label\end{tabular} & \begin{tabular}[c]{@{}l@{}}Median\\ Samples\\ /Label\end{tabular} & \begin{tabular}[c]{@{}l@{}}Max\\ Samples\\/Label\end{tabular} \\ \hline
\textit{eBird} & 100 & 20.69 & 18 & 96 & 8322.95 & 5793 & 29340\\
\textit{bookmarks} & 208 & 2.03& 1& 44 & 584.67 & 381 & 4642 \\
\textit{bibtex}  & 159 & 2.38& 2& 28 & 72.79 & 54 & 689 \\
\textit{mirflickr} & 38 & 4.80 & 5 & 17 & 1247.34 & 799 & 4120\\
\textit{reuters} & 90 & 1.23& 1& 15 & 106.50 & 18 & 2877 \\
\textit{scene} & 6 & 1.07 & 1 & 3 & 170.83 & 168 & 903\\
\textit{sider} & 27 & 15.3 & 16 & 26 & 731.07 & 851 & 1185 \\
\textit{yeast} & 14 & 4.24 & 4 & 11 & 363.14 & 334 & 903
\end{tabular}
}
\end{minipage}
\caption{Dataset Label Statistics. This shows that many samples have more than two labels to be predicted, and each dataset has a varying degree of label density.}
\label{tab:dataset_label_stats}
\end{table}
\end{small}

\paragraph{Baseline Comparisons.}
We compare HOT-VAE with five other state-of-the-art MLC methods.
MLKNN~\cite{zhang2007ml} is a statisical method based on the k-nearest neighbor algorithm.
SLEEC~\cite{NIPS2015_5969} makes no low-rank assumption, and it learns embbeddings perserving pairwise distances between only the nearest label vectors.
C2AE~\cite{yeh2017learning} is a two-branch autoencoder.
It first produces a latent vector for features and a latent vector for labels; then these two latent embedding are associated by deep canonical correlation analysis (DCCA).
seq2seq~\cite{nam2017maximizing} applies a recurrent-neural-neural (RNN) based encoder-to-decoder model where the encoder RNN encodes features and the decoder predicts each positive label sequentially. 
LaMP~\cite{lanchantin2019neural} consists of multiple attention-based neural message passing modules including one sending messages bewteen features, one from features to labels, and one between labels. 
MPVAE~\cite{bai2020disentangled} is a two-branch disentangled VAE building on a covariance-aware multivariate probit model, which can learn pairwise label correlation.

\begin{small}
\begin{table}
\begin{minipage}[h]{.47\textwidth}
\scalebox{0.75}{
\begin{tabular}{@{}c@{\hspace{0.45em}}c@{\hspace{0.45em}}c@{\hspace{0.45em}}c@{\hspace{0.45em}}c@{\hspace{0.45em}}c@{\hspace{0.45em}}c@{\hspace{0.45em}}|c@{}}
Dataset & MLKNN & SLEEC & C2AE & seq2seq & LaMP & MPVAE & ours\\
\hline
\textit{eBird}    & 0.5103 & 0.2578 & 0.5007 & 0.4768 & 0.4768 & 0.5511 & \textbf{0.5747}\\
\textit{bookmarks} & - & - & - & 0.3620 & 0.3551 & - & \textbf{0.3630}\\
\textit{bibtex}    & 0.1826 & 0.4490 & 0.3346 & 0.3930 & 0.4469 & 0.4534 & \textbf{0.4693}\\
\textit{mirflickr} & 0.3826 & 0.4163 & 0.5011 & 0.4216 & 0.4918 & 0.5138 & \textbf{0.5192}\\
\textit{reuters}   & - & - & - & 0.8944 & 0.9060 & - & \textbf{0.9128}\\
\textit{scene}     & 0.6913 & 0.7184 & 0.6978 & 0.7469 & 0.7279 & 0.7505 & \textbf{0.7762}\\
\textit{sider}     & 0.7382 & 0.5807 & 0.7682 & 0.3560 & 0.7662 & 0.7687 & \textbf{0.7708} \\
\textit{yeast}     & 0.6176 & 0.6426 & 0.6142 & 0.5744 & 0.6242 & 0.6479 & \textbf{0.6498}\\


\hline
%\vspace{0cm}
\end{tabular}
}
\end{minipage}
~\\

\begin{minipage}[h]{.47\textwidth}
\scalebox{0.75}{
\begin{tabular}{@{}c@{\hspace{0.45em}}c@{\hspace{0.45em}}c@{\hspace{0.45em}}c@{\hspace{0.45em}}c@{\hspace{0.45em}}c@{\hspace{0.45em}}c@{\hspace{0.45em}}|c@{}}
Dataset & MLKNN & SLEEC & C2AE & seq2seq & LaMP & MPVAE & ours\\
\hline
\textit{eBird}     & 0.5573 & 0.4124 & 0.5459 & 0.5260 & 0.5170 & 0.5933 & \textbf{0.6270}\\
\textit{bookmarks} & - & - & - & 0.3290 & 0.3593 & - & \textbf{0.3682} \\
\textit{bibtex}    & 0.1782 & 0.4074 & 0.3884 & 0.3840 & 0.4733 & 0.4800 & \textbf{0.4823} \\
\textit{mirflickr} & 0.4149 & 0.4127 & 0.5448 & 0.4640 & 0.5352 & 0.5516 & \textbf{0.5559}\\
\textit{reuters}   & - & - & - & 0.8575 & 0.8890 & - & \textbf{0.8910}\\
\textit{scene}     & 0.6667 & 0.6993 & 0.7131 & 0.7442 & 0.7156 & 0.7422 & \textbf{0.7567}\\
\textit{sider}     & 0.7718 & 0.6965 & 0.7978 & 0.3890 & 0.7977 & 0.8002& \textbf{0.8026}\\
\textit{yeast}     & 0.6252 & 0.6531 & 0.6258 & 0.5999 & 0.6407 & 0.6554 & \textbf{0.6595}\\
\hline
%\vspace{0cm}
\end{tabular}
}
\end{minipage}
~\\

\begin{minipage}[h]{.47\textwidth}
\scalebox{0.75}{
\begin{tabular}{@{}c@{\hspace{0.45em}}c@{\hspace{0.45em}}c@{\hspace{0.45em}}c@{\hspace{0.45em}}c@{\hspace{0.45em}}c@{\hspace{0.45em}}c@{\hspace{0.45em}}|c@{}}
Dataset & MLKNN & SLEEC & C2AE & seq2seq & LaMP & MPVAE & ours\\
\hline
\textit{eBird}     & 0.3379 & 0.3625 & 0.4260 & 0.3298 & 0.3806 & 0.4936 & \textbf{0.5350}\\
\textit{bookmarks} & - & - & - & 0.2370 & 0.2939 & - & \textbf{0.2984} \\
\textit{bibtex}    & 0.0727 & 0.2937 & 0.2680 & 0.2820 & 0.3763 & 0.3863 & \textbf{0.3953}\\
\textit{mirflickr} & 0.2660 & 0.3636 & 0.3931 & 0.3333 & 0.3871 & \textbf{0.4217} & 0.4078\\
\textit{reuters}   & - & - & - & 0.4567 & 0.5600 & - & \textbf{0.5748} \\
\textit{scene}     & 0.6932 & 0.6990 & 0.7284 & 0.7490 & 0.7449 & 0.7504 & \textbf{0.7639}\\
\textit{sider}     & 0.6674 & 0.5917 & 0.6674 & 0.2070 & 0.6684 & \textbf{0.6904} & 0.6653\\
\textit{yeast}     & 0.4716 & 0.4251 & 0.4272 & 0.4333 & 0.4802 & 0.4817 & \textbf{0.4885}\\
\hline
\end{tabular}
}
\end{minipage}
\caption{Top: ebF1 scores; Middle: miF1 scores; Bottom: maF1 scores produced by all the methods for each dataset. We mark the best scores with bold texts.}
\label{tab:f1s}
%\vspace{-0.5em}
\end{table}
\end{small}

\paragraph{Other details.}
%We run our model on one NVIDIA Tesla V100 GPU with 16GB memory, or two such GPUs if the model exceeds memory limit of one GPU.
%To obtain best possible performance, we perform grid search on hyperparameters.
%Learning rate is chosen from \{2e-4, 3e-4, 7.5e-4\}; $\lambda_0$ is set to 1; $\lambda_1$ is selected from $\{ 0.1, 0.2, 0.3 \}$; $\lambda_2$ is from $\{ 1, 100, 1000\}$; $\beta$ has a value of 1e-5, or $0$ in some rare cases; $d$ is from \{100, 200, 512\}; and the number of decoder layer is from $\{2,3,4,5\}$.
%We train the model up to 200 epochs to saturate the performance.
We choose two encoders: one is a three-layer MLP which is used for \emph{eBird}, \emph{scene}, \emph{sider}, \emph{sider}, and \emph{yeast}; the other one is a two-layer FMP from \cite{lanchantin2019neural} for the rest of the datasets.
For label graphs, we use both complete graphs and prior graphs (with edges removed if two labels never correspond to any training sample) for each dataset and select the one exhibiting better performance.
Hyperparameter selections and other training details are in the supplementary material.
%To convert the soft predictions into $\{0, 1\}$ values, we use the same thresholds in~\cite{bai2020disentangled} and select the best threshold for each metric.

\subsection{Main Experiments}
\begin{small}
\begin{table}[h]
\scalebox{0.75}{
\begin{tabular}{@{}c@{\hspace{0.45em}}c@{\hspace{0.45em}}c@{\hspace{0.45em}}c@{\hspace{0.45em}}c@{\hspace{0.45em}}c@{\hspace{0.45em}}c@{\hspace{0.45em}}|c@{}}
Dataset            & MLKNN  & SLEEC & C2AE   & seq2seq & LaMP            & MPVAE & ours          \\
\hline
\textit{eBird}     & 0.8273 & 0.8156 & 0.7712 & 0.8236 & 0.8113 & 0.8286 &\textbf{0.8455}\\
\textit{bookmarks} & - & - & - & 0.9900 & \textbf{0.9917} & - & \textbf{0.9917}        \\
\textit{bibtex}    & 0.9853 & 0.9818 & 0.9867 & 0.9850 & 0.9876 & 0.9875 & \textbf{0.9878}        \\
\textit{mirflickr} & 0.8767 & 0.8698 & 0.8973 & 0.8839 & 0.8969          & 0.8978 & \textbf{0.8980}\\
\textit{reuters}   & - & - & - & 0.9962 & 0.9970 & - & \textbf{0.9971}          \\
\textit{scene}     & 0.8633 & 0.8937 & 0.8934 & \textbf{0.9456} & 0.9025          & 0.9094 & 0.9155\\
\textit{sider}     & 0.7146 & 0.6750 & 0.7487 & 0.5930 & 0.7510          & 0.7547 & \textbf{0.7555}\\
\textit{yeast}     & 0.7835 & 0.7824 & 0.7635 & \textbf{0.8177} & 0.7857          & 0.7920 & 0.7947\\

\hline
\end{tabular}
}
\caption{HAs for all the methods on each dataset.}
\label{tab:ha}
\end{table}
\end{small}

\begin{table*}[t!]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|cccc|cccc|cccc}
        & \multicolumn{4}{c|}{Occurrences}                                           & \multicolumn{4}{c|}{Richness}                                           & \multicolumn{4}{c}{Community}                                                                                                                 \\ \cline{2-13}
        & Accuracy        & Discrimination  & Calibration     & Precision       & Accuracy         & Discrimination  & Calibration     & Precision       & Accuracy                          & Discrimination                    & Calibration                       & Precision                         \\ \hline
MPVAE   & 0.3093          & 0.7803          & 679.8019        & 0.3772          & 18.3679          & 0.4425          & 0.4198          & 4.0185          & (0.2208, 0.2443, 0.2318)          & (0.4053, 0.1910, 0.0502)          & (0.3067, 0.3340, 0.3367)          & \textbf{(0.0708, 0.0842, 0.0373)} \\
HOT-VAE & \textbf{0.2062} & \textbf{0.8278} & \textbf{124.96} & \textbf{0.2612} & \textbf{10.8392} & \textbf{0.6279} & \textbf{0.2679} & \textbf{3.0248} & \textbf{(0.1512, 0.2268, 0.1727)} & \textbf{(0.5549, 0.4326, 0.3509)} & \textbf{(0.2033, 0.2233, 0.2633)} & (0.0831, 0.1214, 0.0668)         
\end{tabular}%
}
\caption{HOT-VAE vs. MPVAE on 12 ecological metrics. For accuracy, calibration, and precision, scores are the smaller, the better; for discrimination, scores are the larger, the better. The better scores are marked with bold texts.}
\label{tab:eco}
\end{table*}

In Table~\ref{tab:f1s}, we present the main experimental result evaluated on three F1-scores: example-based F1 (ebF1), micro-averaged F1 (miF1), and macro-averaged F1 (maF1).
%They are calculated from the precision and recall of the predictions, where precision measures how many positive labels are correctly identified in all the predicted labels, and recall measures how many positive labels are correctly identified in all ground-truth labels.
F1-score is the harmonic mean of precision and recall of the predictions.
ebF1 is the average of the F1-score for each test sample.
miF1 aggregates total true positives, false negatives, and false positives for all class labels, and computes a F1-score.
maF1 computes the F1-score independently for each class and returns the average with equal weights for all classes.
Larger F1-scores indicate better performance, with the highest possible value being 1, meaning perfect precision and recall.
We note that high ebF1s show strong results over all test samples, high miF1s indicate strong performance on the most frequent labels, and high maF1 implies strong performance on less frequent labels.
We select the model performing best on validation set based on maF1.

We note that \emph{reuters} deals with sequential input and \emph{bookmarks} has over 380 thousand features; hence, we only compare to seq2seq and LaMP, which can handle position information or inputs with extremely high dimensions.
HOT-VAE outperforms all the baseline approaches on ebF1, yielding a 2.13\% improvement to MPVAE and a 5.69\% improvement to LaMP on average.
Our model again produces the best performance within all the methods on miF1, improving MPVAE by 1.63\% and LaMP by 4.88\% on average.
HOT-VAE performs less well for predicting the rare labels on \emph{sider} and \emph{mirflickr}, indicated by maF1, but it still produces an improvement on most of the datasets.

We also test HOT-VAE on Hamming accuracy (HA), which measures how many labels are correctly predicted in all the labels regardless of being positive/negative.
Table~\ref{tab:ha} summaries the HAs of all the methods on each dataset.
seq2seq performs better than HOT-VAE on \emph{scene} and \emph{yeast}, because they directly maximize subset accuracy, and this works well when the number of labels is small.
Otherwise, HOT-VAE has the best HAs.

\subsection{Measuring Predictive Performance on Species}
% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=0.45\textwidth]{figs/eco1.pdf}
%     \caption{HOT-VAE vs. MPVAE on 12 ecological metrics. X-axis shows each group of measures. Y-axis is MPVAE's score divided by HOT-VAE's score. Thus, a bar above y=1 means HOT-VAE has a lower score than that of MPVAE for the corresponding metric, and vice versa.}
%     \label{fig:eco}
% \end{figure}



%One important question to ask is whether HOT-VAE produces meaningful improvements that an ecologist cares about.
%In order to conduct a comprehensive evaluation on species prediction, \citet{norberg2019comprehensive} propose 12 measures for the biological levels of species occurrences, species richness, and community composition.
%Species occurrences measure a model's performance for predicting presence/absence of individual species occurrences; species richness regards to predicting the number of species for a given location; and community composition evaluates whether presence/absence of species groups can be correctly identified.
%For analyzing each level, four statistical metrics are applied: accuracy, calibration, precision, and discrimination power of predictions.
%We compare our model to MPVAE, the best-performing baseline method on \emph{eBird}.

%We present the experimental result for the 12 measures in Figure~\ref{fig:eco}.
%For each metric, y-axis shows the ratio of MPVAE's score to HOT-VAE's score.
%Scores for all the measures are the lower the better (we show the exact calculations of these values in supplementary materials).
%A bar higher than y=1 means our score is lower than that of MPVAE; the more a bar is higher than y=1, the better performance it indicates.
%Of the 12 measures, we only have worse precision at the community composition level; this is because community composition only considers pairs, and MPVAE is optimized for modeling pair relation.
%We substantially outperform MPVAE on almost all other metrics.

Ecologists use joint species distribution models for a number of distinct applications.
To determine if HOT-VAE produces ecologically meaningful improvements in model performance we evaluated the 12 metrics presented in Norberg et al. (2019) used to assess performance predicting species occurrences, species richness, and community composition.
The occurrence metrics measure a model’s performance for predicting presence/absence of individual species, the richness metrics measure the ability to predict the total number of species that occur at a given location and time, and the community metrics measure the ability to predict species occurrences at location pairs.
Four metrics are applied for predicting each of species occurrences, species richness, and community composition: accuracy, calibration, precision, and discriminative power of predictions. We compare our model to MPVAE, the best performing baseline method on \emph{eBird}.

The experimental results for the 12 measures are shown in Table~\ref{tab:eco}.
%For each metric, y-axis shows the ratio of the MPVAE score to the HOT-VAE score.
%For all 12 measures, lower is better.
For accuracy, calibration, and precision, smaller values indicate better predictive performance; for discrimination power, larger values are better (calculations of these values are in supplementary material).
%Ratios greater than one indicate where HOT-VAE outperforms MPVAE.
HOT-VAE outperforms MPVAE for 11 of the 12 metrics.
We only have worse precision at the community composition level; this is because this community composition metric only considers pair-wise co-occurrence of species, and MPVAE is optimized for modeling interactions specifically between pairs of species.


\subsection{Ablation Studies}
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.45\textwidth]{figs/ndec.pdf}
    \caption{maF1 scores for the datasets \emph{ebird}, \emph{mirflickr}, \emph{bookmarks} when the number of decoder layers increases.}
    \label{fig:ndec}
\end{figure}
We further investigate how incorporating high-order label correlation impacts predictive performance.
We postulate that, for learning $n$-order label correlation, increasing $n$ would be particularly beneficial for improving predictions of rare labels: when treating classifying each label as individual problem, there is very limited information to learn from for the rare labels; including higher-order interactions between labels provides much additional information to a model.

To verify this hypothesis, we train HOT-VAE with different numbers of decoder layers and see how maF1 scores vary under these settings, as high maF1 scores indicate strong results on less frequent labels.
We select three datasets \emph{ebird}, \emph{mirflickr}, and \emph{bookmarks}, which have median labels 18, 5, and 1, respectively.
In Figure~\ref{fig:ndec}, we show maF1 scores for these datasets at $n$ being 1-5.
For the datasets with more labels per sample, larger $n$ has more positive impacts on maF1 scores.
It is also possible increasing $n$ beyond some threshold negatively affects performance as the model may start to overfit.
In general, for the datasets with dense labels, having $n=4,5$ produces best results.
After that, we are likely to hit diminishing returns. 

\begin{small}
\begin{table}[t!]
\centering
\scalebox{0.6}{
\begin{tabular}{c|cccccccc}
         & \emph{mirflickr}       & \emph{ebird}           & \emph{scene}           & \emph{yeast}           & \emph{reuters}         & \emph{sider}           & \emph{bookmarks}       & \emph{bibtext}         \\ \hline
prior    & \textbf{0.8169} & \textbf{0.8259} & \textbf{0.9471} & 0.6857          & \textbf{0.9915} & \textbf{0.5151} & 0.9162          & 0.9405          \\
complete & 0.8116          & 0.8251          & 0.9355          & \textbf{0.6869} & 0.9882          & 0.5120          & \textbf{0.9192} & \textbf{0.9457}
\end{tabular}
}
\caption{medianAUC for each dataset when decoder is on a complete label graph and on a prior label graph.}
\label{tab:prior}
\end{table}
\end{small}

Additionally, we evaluate the effect of incorporating prior knowledge.
We train HOT-VAE on both complete label graphs and prior label graphs, in which we remove the edges between the label pairs if they never positively correspond to any training sample.
To have one metric summarizing the overall performance, we use medianAUC (described in the supplementary material), which represents the probability that a random positive sample is ranked higher than a random negative sample.
In Table~\ref{tab:prior}, we show medianAUC for each dataset when HOT-VAE is trained with these two label graphs respectively.
We see that using prior graphs slightly improves predictive performance in many cases and is at least comparable to using complete graphs in all cases.



==> hot-vae arxiv/introduction.tex <==
% state the 
% focus on higher order reasoning, give examples
% condition on input
% easily incorporate prior knowledge
\section{Introduction}
%\SK{Start talking with tasks in ecology, what's the challenges, why's that important, and these challenges led to what problems in computer science with particular constraints or requirements. Then talk about what's the limitations of current techniques in CS to address these challenges, and your methods to address these limitations. See https://www.ijcai.org/Proceedings/2020/0603.pdf for an example.}

The study of multi-label classification (MLC) is an active research area and has been receiving increasing attention in the past few decades; unlike traditional single-output learning, it is a task of predicting the presence and absence of multiple entities simultaneously given a sample with a set of features.
It finds applications in a wide range of domains including image recognition, natural language processing, and bioinformatics~\cite{8892612}.

One important field that is in urgent need for a scalable and accurate MLC approach is ecology.
The ability to accurately predict which species assemble into communities based on local environmental features is essential to understand how changes in the environment can be expected to impact biodiversity and to plan for the restoration and recovery of species communities in the face of environmental change~\cite{d2017spatial}.
This problem is represented as joint species distribution modelling (JSDM), which predicts species occurrences given environmental features and species interactions.
There are two key challenges in JSDM.
First, species communities are often comprised of very large numbers of individual species, presenting the challenge of learning complex high-dimensional interactions.
For example, bird communities are often comprised hundreds of individual species within a single region.
To consider how all subsets of all bird species interact is computationally intractable, thus being selective in how we model these interactions is a necessity.
On one hand, accounting for more interactions increases learning capacity but will be more computationally demanding and could have a higher risk of over-fitting.
On the other hand, one can focus on less or no interactions; however, many communities of species are known to include complex interactions among large numbers of species, so having oversimplifying assumptions leads to inaccurate predictions.
The second challenge for modeling the joint distribution of many species is the fact that the relationships between species change as important features of the environment change over space and time.
Thus, it is critical to understand how environment changes like climate change impact species interactions and the resulting structure of species communities~\cite{evans}.

%One important field that is in urgent need for a scalable and accurate MLC approach is ecology:
%To promote biodiversity and prevent species from going extinct, a better understanding of how species interact with each other is beneficial for adaptive management for species recovery~\cite{evans}.
%Several challenges have arisen for performing joint species modelling effectively.
%First of all, correlations between species may be different as the environmental factors change over time, as \citet{evans} has identified that climate change exacerbates species monitoring and thus increases management uncertainty.
%It is then critical to capture how environment changes impacts on species interactions.
%Secondly, there is often a large number of species to be predicted, and the ability to model their interactions is essential for accurate predictions.
%For example, in a bird distribution dataset~\cite{munson2012ebird}, the classification is for over a thousand bird species.
%To consider how all subsets of all bird species interact results is computationally intractable, thus being selective is a necessity.
%On one hand, taking into account more interactions leads to a stronger capacity to learn but will be  computationally demanding and may have the risk of over-fitting.
%On the other hand, one can focus on less or no interactions; however, in a real world species correlations are complex, and having oversimplifying assumptions leads to inaccurate predictions.
%Finally, representing and making efficient use of domain knowledge can be crucial to improve performance when it is available.
%Therefore, a method that efficaciously overcomes these challenges will illuminate a path to better protect biodiversity.

\textbf{Our contributions:} We propose High-order Tie-in Variational Autoencoder (HOT-VAE), an attentioned-based VAE that leverages latent embedding learning and neural message passing to perform high-order label correlation learning and produce accurate multi-label predictions. More specifically:
(1) We introduce a two-branch VAE-based model with a replaceable, domain-specific encoder (i.e., one can choose an encoder that efficiently extracts feature information given an application domain) and a shared message passing neural network (MPNN) decoder where label correlations are computed.
(2) HOT-VAE is able to learn high-order label correlation using multiple-step message passing. It also produces label correlation conditioned on features. In other words, HOT-VAE can not only model the interactions between many species simultaneously, it can  also adapt the correlation between species to changing environmental factors.
(3) With a graph structure to reason about label correlation, we can easily incorporate prior knowledge, resulting in better empirical results.
(4) We perform thorough experimental evaluations on a JSDM dataset and seven other real-world datasets on a variety of metrics, and we show HOT-VAE outperforms (or is comparable to) other state-of-the-art MLC methods. On the JSDM dataset, we further evaluate HOT-VAE on several ecological metrics; the result suggests that HOT-VAE produces a meaningful improvement in the field of ecology.

==> hot-vae arxiv/method.tex <==
\section{Method: Attention-based VAE \\ for High-order Correlation}

% There are three message passing modules, and we first look at sending messages from feature to feature used to model interactions between features.
% We define a feature graph $G_{xx}=(V_{xx}, E_{xx})$ where $V_{xx}=\{x_{k}|1\leq k \leq S \}$ and $G_{xx}$ is fully connected unless some prior structure on features is known.
% We denote the message passing module by $\textrm{MPNN}_{xx}$, parameterized by $\textbf{\textrm{W}}_{xx}$.
% LaMP uses embedding vectors $\{ \textbf{z}^t_1,\textbf{z}^t_1, ..., \textbf{z}^t_S \}$ to represent nodes and the initial states are obtained from feature embedding $\textbf{W}^x \in \mathbb R^{S \times d}$.
% $\{\textrm{z}^t_{1:S}\}$ is updated as follows:

% \begin{gather}
%     \bm{m}^t_i = \bm{z}^t_i + 
%     \sum_{j \in \mathcal{N}(i)} M_{\textrm{atn}}(\bm{z}^t_i,\bm{z}^t_j; \bm{W}_{\textrm{xx}}), \\
%     {\bm{z}}^{t+1}_i = \bm{m}^t_i + U_{\textrm{x}}(\bm{m}^{t}_i; \bm{W}_{\textrm{xx}}).
% \end{gather}

%The MPNN in the encoder operates on features, where a feature is a node, and every feature is connected to every other feature unless some prior structure about the features is known.
%Similarly, the MPNN in the decoder operates on the label graph.
% MPNN operates on a graph $(V,E)$ where $V$ is a set of nodes representing objects and $E$ is a set of edges describing how objects interact with each other.
% On a high level, at each update step, a node $v_i$ collects information from its neighborhood (the nodes that have an edge to $v_i$), so that an update depends on itself as well as its neighbors.
% Compared to probabilistic classifier chain methods~\cite{wang2016cnn,nam2017maximizing} where the joint probabilities of labels are explicitly modelled using chain rules, MPNNs use message passing to implicitly mimic this process, thus allowing fast inference and parallel computation.

% Formally, MPNNs run in two phases: a message passing phase and a readout phase.
% The message passing phase has a total of $T$ update steps and is defined in terms of message function $M_t$ and node update function $U_t$.
% At each time step, hidden state $v_i^t$ of node $v_i$ at time $t$ is updated according to

% \begin{equation}
%     m_i^t = \sum_{j \in N(i)} M_t(v_i^t, v_j^t, e_{ij}),
% \end{equation}
% \begin{equation}
%     v_i^{t+1} = U_t(v_i^{t}, m_i^t)
% \end{equation}

% Next, a readout phase is executed to make predictions such as classifying the nodes or outputting the graph properties.
% A readout function $R$ runs as follows:

% \begin{equation}
% \hat{y} = R(\{v_i^T | v_i \in V \})
% \end{equation}

% We note that $M_t$, $U_t$, and $R$ are differentiable, and the output of $R$ is invariant to any permutation of nodes, preserving graph isomorphism.

% There are many choices existed for $M_t$ and $U_t$.
% \citet{lanchantin2019neural} use self-attention (also known as intra-attention) neural message passing, which we will be following in this work.
% Attention is originally proposed for seq2seq models in the field natural language processing~\cite{bahdanau2014neural, luong2015effective}.
% Intuitively, attention enables the model to focus on the relevant parts of the input as needed.
% In the case of a label graph, attention allows a label node to attend its neighborhood differentially; in other words, some label nodes contribute more to predicting the presence/absence of the label than other label nodes do.
% To compute self-attention on a MPNN, we calculate attention weight for each node pair $(v_i^t, v_j^t)$ by attention function $a(\cdot)$

% \begin{align}
%     \alpha^t_{ij} = \textrm{softmax}_j(e^t_{ij}) &=  \frac{\textrm{exp}(e^t_{ij})}{\sum_{k \in \mathcal{N}(i)}{\textrm{exp}(e^t_{ik})}} \label{eq:alpha}
% \end{align}

%\subsection{\TODO{NAME} Networks}

\begin{figure*}
  \centering
  \includegraphics[width=0.45\textwidth]{figs/modelarch.png}
  \includegraphics[width=0.45\textwidth]{figs/decoder.png}
  \caption{Model architecture of HOT-VAE. (A): Overall network architecture. The feature encoder maps features $x$ to a set of probabilistic latent subspaces using a neural network parameterized by $\psi$. Similarly, the label encoder with parameter $\phi$ maps labels $y$ to another set of probabilistic latent subspaces. Then, sampled from their own distributions, $\{z_{x}^{(j)}\}$ and $\{z_{y}^{(k)}\}$ are separately fed into a shared decoder. Finally, for the feature branch, the decoder outputs label prediction $\hat{y}_f$, and for the label branch, the decoder outputs reconstruction $\hat{y}_l$. At inference, only the feature branch is used. (B): The shared decoder is a graph with each node being a label. An edge is connecting two nodes if we believe correlation exists between them. By default, there is an edge between every pair of labels. The figure shows all the other nodes are sending messages to the $y_1$ node with learned attention weights $e$. (C): Decoder layers. At each layer, masked multi-head self-attention is computed and goes through a feed-forward operation. $n$ is the number of layers. We note that these layers are shared by all label nodes.}
  \label{fig:model}
\end{figure*}

%MPVAE uses aligned two-branch VAEs to impose label-aware structure on the feature latent space, such that the feature latent space represents both input features and output labels, which could further help the task of label prediction. However, the shared decoder of MPVAE is the multivariate probit (MVP) model.
%It is unclear how the MVP model could  reason about high-order label correlation or incorporate prior knowledge.
%Moreover, LaMP does not utilize labels to help with learning feature embedding, which has been shown to be beneficial to classification performance~\cite{yeh2017learning}.
%In order to address the limitations in MPVAE and in LaMP
We propose HOT-VAE, a novel two-branch variational autoencoder model building on top of attention-based neural message passing networks for MLC, which can learn feature embeddings representing both input features and output labels, perform high-order correlation learning, and flexibly incorporate prior knowledge on label structures.
The illustration of the framework is shown in Figure~\ref{fig:model}.
At training, the feature encoder and the label encoder first map features and labels to a set of Gaussian subspaces respectively.
There are many possible ways to parameterize the encoders; common choices are multi-layer perceptrons and graph networks such as graph convolutional networks and message passing neural networks.
Then, the shared decoder makes a prediction on labels based on the samples from the feature Gaussian subspace and recovers the input labels based on the samples from the label Gaussian subspace.
There are two message passing modules.
One passes attention from features to labels, and the other passes attention from labels to labels.
%We note that only the feature branch is needed for inference.
%The key to make a connection between two branches is the alignment operation to match two sets of Gaussian subspaces.

\subsection{Learning and Aligning Probabilistic Subspaces}
We assume that both the feature embedding and the label embedding have $d$ dimensions.
If each encoder only outputs one Gaussian subspace, in the case of it being an MLP, $\mathcal D[q_\phi(\textbf{z}|\textbf{y})||q_\psi(\textbf{z}|\textbf{x})]$ is simply the KL divergence between two multivariate normal distributions.
Since both distributions have diagonal covariance matrices, we can derive the KL divergence to be the following:
\begin{small}
\begin{equation}\label{eq:kl}
\begin{split}
    \mathcal{L}_{\text{KL}}(\bm{x},\bm{y})=&\beta[\sum_{i=1}^d\log\frac{\Sigma^\psi_{i,i}(\bm{x})}{\Sigma^\phi_{i,i}(\bm{y})}-d+\sum_{i=1}^d\frac{\Sigma^\phi_{i,i}(\bm{y})}{\Sigma^\psi_{i,i}(\bm{x})}+\\
    &\sum_{i=1}^d\frac{(\mu^\psi_i(\bm{x})-\mu^\phi_i(\bm{y}))^2}{\Sigma^\psi_{i,i}(\bm{x})}]
\end{split}
\end{equation}
\end{small}
However, there are features which MLPs cannot encode, such as English texts and graphs.
To have a general multi-label classifier, encoders need to be flexible with regards to network architecture to deal with different types of inputs.
Then, it becomes possible that the feature encoder and the label encoder output different numbers of Gaussian subspaces.
For example, if we adopt the Transformer encoder~\cite{vaswani2017attention} to be the feature encoder and the label encoder, the two encoders may generate two sets of Gaussian subspaces of varying sizes.
This is because for every dimension of the input, a mean and a variance are computed, and features and labels often differ in their dimensionality.
For example, let us consider when the input text is seven words - ``my favorite football player lost a game'' and the labels are ``sad'' and ``angry''.
The feature transformer outputs one Gaussian subspace for each of the seven words, and the label transformer outputs two subspaces.
%Further, we note that since the number of features may vary from samples to samples (e.g., classifying sentences of different numbers of words), hard-coding a projection mapping from a fixed number of Gaussian subspaces to match the size of label Gaussian subspaces would not work.
To overcome this issue, suppose the feature encoder outputs $J$ subspaces and the label encoder outputs $K$ subspaces, we compress $J$ subspaces and $K$ subspaces into one subspace by computing a mean vector for $\mu$ and for $\Sigma$, respectively.
Formally, $\mu^\psi(\bm{x})$ and $\Sigma^\psi(\bm{x})$ now become:
\begin{align}
    \mu^\psi{(\bm{x})} &= \frac{1}{J}\sum_{j=0}^{J-1} \mu^\psi(\bm{x})^{(j)}\\
    \Sigma^\psi{(\bm{x})} &= \frac{1}{J}\sum_{j=0}^{J-1} \Sigma^\psi(\bm{x})^{(j)}
\end{align}
And we do the same for $\mu^\phi(\bm{y})$ and $\Sigma^\phi(\bm{y})$.
With these operations, we can again use Equation~\ref{eq:kl} to compute the divergence between two probabilistic latent spaces.
It is worth noting that because there is not a one-to-one relationship from one feature Gaussian subspace to one label Gaussian subspace, there is no point in aligning individual feature subspaces to individual label subspaces.

Lastly, although we collapse all Gaussian subspaces into a unified one to compute alignment, we still feed unmodified $\{\bm{z}^{(j)}_{\bm{x}}\}$ and $\{\bm{z}^{(k)}_{\bm{y}}\}$ into the shared decoder to keep as much information as possible.
%difficult that label branch and feature branch output different sizes
%compute mean
%but still feeds all the node information into decoder

\subsection{Learning High-Order Label Correlation}
We highlight three features of the shared decoder:
(1) The decoder computes the correlation between labels conditioned on features $\bm{x}$; thus, the label correlation becomes sensitive to changes in $\bm{x}$, which enables adaptive learning for label interactions.
(2) With the label graph, one can easily impose prior structure between labels by adding and removing edges. If it is known in advance two labels are independent from each other, then leaving out the edge connecting these two label nodes prevents the model from over-fitting and learning noise.
(3) Most importantly, the decoder is able to capture higher-order label correlation in a scalable way, as opposed to PCC methods~\cite{wang2016cnn,nam2017maximizing} where chain rules are used to model the joint probabilities of labels.

We now turn to a detailed description of HOT-VAE's decoder.
Labels are represented as embedded vectors $\{\bm{u}^t_1, \bm{u}^t_2, \dots, \bm{u}^t_L\}$, where $\bm{u}^t_i \in \mathbb R^d$ and initial $\bm{u}^{t=0}_i$ is obtained from a learnable embedding matrix $\textbf{W}^{y} \in \mathbb R^{L \times d}$.
Figure~\ref{fig:model}(C) shows an overview of the decoder layers.
Self-attention is computed based on Equations~\ref{eq:alpha}-\ref{eq:mt}, and feed forward is computed using Equation~\ref{eq:u_attention}.
Specifically, we use multi-head self-attention~\cite{vaswani2017attention}, so that a node can attend to multiple other nodes at once.
We also apply layer normalization~\cite{ba2016layer} around each of the attention and feedforward sublayers to alleviate training issues.
After the $n$'s layers (thus $\bm{u}^{t=0}_i$ becoming $\bm{u}^t_n$), a readout layer predicts each label $\hat{y}_i$, where a readout function $R$ projects $\bm{u}_i^{n}$ using a projection matrix $\textbf{W}^o \in \mathbb R^{d\times d}$.
The $i$th row of $\textbf{W}^o$ is denoted by $\textbf{W}^o_i$.
The resulting vector of size $L \times 1$ is then fed through an element-wise sigmoid function to produce the final probabilities of all labels:
\begin{equation}
   \label{eq:readout}
    \hat{y}_i = R({\bm{u}}^n_i;{\textbf{W}^o}) = \textrm{sigmoid}({\textbf{W}^o_i} {\bm{u}}^n_i).
\end{equation}

As mentioned above, to pass the message from encoder to decoder, 
we feed unmodified $\{\bm{z}^{(j)}_{\bm{x}}\}$ and $\{\bm{z}^{(k)}_{\bm{y}}\}$ into the shared decoder to keep as much information as possible.
For clarity, we look at the feature branch, and the label branch works similarly.
We denote the message passing module from $\{ {\bm{z}^{(j)}_{\bm{x}}} \}$ to label nodes by $\bm{W}_{\textrm{fy}}$ and the message passing module between label nodes by $\bm{W}_{\textrm{yy}}$.
We compute the initial state $\bm{u}^{t'}_i$ of the decoder w.r.t. the feature branch as:
%Looking at how samples $\{ {\bm{z}^{(j)}_{\bm{x}}} \}$ are passed into the decoder at the feature branch,
\begin{gather}
    \bm{m}^t_i = \bm{u}^t_i + 
    \sum\limits_{j=1}^J M_{\textrm{atn}}(\bm{u}^t_i,\bm{z}^{(j)}_{\bm{x}}; \bm{W}_{\textrm{fy}}), \\
    \bm{u}^{t'}_i = \bm{m}^t_i + U_{\textrm{mlp}}(\bm{m}^{t}_i; \bm{W}_{\textrm{fy}}).
\end{gather}

After $\bm{u}^{t}_i$ is updated to $\bm{u}^{t^\prime}_i$ with feature information, the message passing between labels then begins,

\begin{gather}
    \label{eq:label_to_label_M}
    \bm{m}^{t'}_i = \bm{u}^{t'}_i + 
    \sum_{l \in \mathcal{N}(i)} M_{\textrm{atn}}(\bm{u}^{t'}_i,\bm{u}^{t'}_l; \bm{W}_{\textrm{yy}}), \\
    {\bm{u}}^{t+1}_i = \bm{m}^{t'}_i + U_{\textrm{mlp}}(\bm{m}^{t'}_i; \bm{W}_{\textrm{yy}}).
\end{gather}

%Therefore, this update scheme ensures the label correlation takes into account the feature information.

We can also incorporate prior knowledge for label-to-label message passing by simple pre-processing: starting from a complete label graph where every node is connected to every other node, we can remove the edge between a pair of nodes if they never belong to any sample simultaneously in the training set.
Depending on a dataset's domain, additional expert knowledge from the domain can be enforced on a dataset-to-dataset basis.
For instance, for predicting species distribution, one can incorporate evolutionary relationships between species, often represented as tree-structures~\cite{ovaskainen2017make,letunic2007interactive}.

%Lastly, it is clear that each self-attention layer learns its label correlation based on the previous one, so stacking $n$ such layers enables us to learn the desired high-order label correlation in the last self-attention layer.

% \begin{wrapfigure}{i}{0.25\textwidth}
%   \begin{center}
%     \includegraphics[width=0.25\textwidth]{figs/highorder.png}
%   \end{center}
%   \caption{Birds}
% \end{wrapfigure}

%\begin{comment}
\begin{figure}
  \begin{center}
    \includegraphics[width=0.25\textwidth]{figs/highorder.png}
  \end{center}
  \caption{An example of higher-order correlation between labels. $u_i^t$ is the hidden representation of $y_i$ at time $t$. The figure shows how correlation is formed within the label triplets $\{ y_2, y_3, y_1 \}$ and $\{ y_2, y_3, y_4 \}$.}
  \label{fig:highorder}
\end{figure}

Finally, we describe how HOT-VAE learns higher-order correlation between labels.
If there is a single layer in the decoder, then messages are passed once from labels to labels, which computes correlation between any pair of labels.
Going to higher order, we only need to increase the number of layers in the decoder.
$n$ times of message passing between labels enable learning $(n+1)$-order label correlation.
In Figure~\ref{fig:highorder}, we present a visual explanation, showing how correlation is learned for two label triplets $\{ \bm{y}_2, \bm{y}_3, \bm{y}_1 \}$ and $\{ \bm{y}_2, \bm{y}_3, \bm{y}_4 \}$.
In this example, at time $t-1$, label 3 collects information from labels 1, 4.
At time $t$, label 2 further collects information from label 3.
By this time, two paths has been built from $1\rightarrow3\rightarrow2$ and $4\rightarrow3\rightarrow2$.
Therefore, the presence of label 2 conditions on the label pairs (1, 3) and (4, 3).
This can be easily extended to high orders.
%\end{comment}

\begin{comment}
\paragraph{Sharing Label Embedding Weights.}
The learned label embedding matrix $\textbf{W}^{y}$ is shared in three places: producing the input to the label encoder (with one exception when it is an MLP, we input labels directly), producing input to the shared decoder, and used as the readout projection matrix (i.e., $\textbf{}{W}^{o} \equiv \textbf{}{W}^{y}$).
The benefits are that $\textbf{W}^{y}$ have more chances to learn and update itself by being in multiple places, and that it also enforces each label's embedding correspond to that particular label
\cite{press2017using}.
\end{comment}

\subsection{Loss Function}
The whole model can be trained in an end-to-end fashion with the Adam optimizer~\cite{DBLP:journals/corr/KingmaB14}.
The overall loss function consists of four parts.
We denote the true binary label vector by $\bm{y}$.
For both the feature and the label branches, we compute binary cross entropy (BCE) over all outputs $\bm{y}_i$ for every sample:
\begin{equation}
    \mathcal{L}_{\textrm{BCE}} = (BCE(\bm{y},\hat{\bm{y}}_f) + BCE(\bm{y},\hat{\bm{y}}_l))
\end{equation}
where BCE is defined by:
\begin{equation*}
    \label{eq:bce_loss}
    BCE(\bm{y},\hat{\bm{y}}) = \frac{1}{L}\sum_{i=1}^{L} -(y_i\log(\hat{y}_i)+(1-y_i)\log(1-\hat{y}_i)) 
\end{equation*}

Further, since the decoder iteratively updates the label node from $t=0$ to $n$, we can also pass those intermediate states from $t=1$ to $n-1$ through a readout layer and enforce BCE loss on these states.
\begin{equation}
    \mathcal{L}_{\textrm{INT}} = (\sum_{t=1}^{n-1} BCE(\bm{y},\hat{\bm{y}}_f^t) + \sum_{t=1}^{n-1} BCE(\bm{y},\hat{\bm{y}}_l^t))
\end{equation}

We also include ranking loss~\cite{6471714} defined as follows, which is shown beneficial in many multi-label tasks:

\begin{equation*}
    RL(\bm{y},\hat{\bm{y}}) = \frac{1}{|{Y}||\bar{{Y}}|} \sum_{(r,s) \in (Y, \bar{Y})} \textrm{exp}(-\hat{y}_r-\hat{y}_{s})
\end{equation*}

where $Y$ is the set of indices for true positive labels and $\bar{Y}$ is the set of indices for true negative labels. $\hat{y}_r$ and $\hat{y}_s$ are the corresponding $r$-th and $s$-th probabilities outputted by the model.
The ranking loss penalizes when a relevant label to the sample is ranked higher than an irrelevant label.
Again, the ranking loss is calculated for both two branches:

\begin{equation}
    \mathcal{L}_{\textrm{RANK}} = (RL(\bm{y},\hat{\bm{y}}_f) + RL(\bm{y},\hat{\bm{y}}_l))
\end{equation}

Finally, with the KL divergence computed for the two branches included, the overall loss function becomes:
\begin{equation}
    \mathcal{L} = \lambda_0 \mathcal{L}_{\textrm{BCE}} + \lambda_1 \mathcal{L}_{\textrm{INT}} + \lambda_2 \mathcal{L}_{\textrm{RANK}} +\beta \mathcal{L}_{\textrm{KL}}
\end{equation}
$\lambda_0, \lambda_1, \lambda_2$ and $\beta$ controls the weights of the four loss terms.



==> hot-vae arxiv/related.tex <==
\section{Related Work}

%Methods of MLC fall into three categories concerning how to represent and model complex interactions among labels~\cite{6471714}: 
%(1) disregarding any relevance among labels and treat a MLC problem as a number of independent binary classification problems~\cite{boutell2004learning,zhang2007ml},
%(2) considering pairwise label correlations~\cite{qi2007correlative,chen2018end,bai2020disentangled},
%and (3) employing various high-order strategies such as collecting all other labels' information for each label~\cite{yan2007model, cheng2009combining} and randomly including correlations within subsets of labels~\cite{read2011classifier}.
%However, they do not consider label correlations that goes beyond second order and cannot systematically incorporate prior knowledge.

We discuss three groups of MLC methods and how they are related to our approach.
The first group is binary relevance (BR) methods which treat a MLC problem as a number of independent binary classification problems~\cite{boutell2004learning,zhang2007ml}.
To add label correlation, probabilistic classifier chains (PCCs) stack binary classifiers sequentially and output one label at a time conditioned on all previously predicted labels~\cite{read2008multi,cheng2010bayes}.
%There are emerging efforts in applying recurrent neural network (RNN) modules to reason about the high-order label correlations.
Followup works extend PCCs to recurrent neural networks~\cite{wang2016cnn,nam2017maximizing}.
%\citet{wang2016cnn} stacks the prediction of each label into an RNN chain, and therefore the predictions of future labels are conditioned on the probabilities of previous labels.
%\citet{nam2017maximizing} reduces the label powerset complexity by only considering the label correlations among positive labels and utilizes the seq2seq RNN model with one RNN encodes features and another RNN to output labels sequentially.
This group suffers from two issues: the quality of predictions can be highly dependent on label ordering, and the nature of autoregressive models prohibits them from parallel computation.

The second group deals with latent embedding, in which they learn one shared latent space representing both input features and output labels~\cite{bhatia2015sparse,yeh2017learning,tang2018multi,chen2019two}.
Most recently, \citet{bai2020disentangled} propose MPVAE: it learns VAE-based probabilistic latent spaces for both labels and features and aligns the latent representations using the Kullback–Leibler divergence.
%; then, it uses a shared decoder to decode the sample from the label subspace to reconstruct the original labels and to decode the sample from the feature subspace to make predictions.
These methods impose label-aware structure on the feature latent space, which is empirically showed to produce better predictive performance.
However, they only consider up to second-order label correlation: MPVAE's decoder is an multivariate probit model (MVP)~\cite{chen2018end} which employs a covariance matrix on labels to capture pairwise relations, and \citet{bhatia2015sparse} find k-nearest neighbors for label embeddings.
Another limitation is that these label correlations are global: when features change, the label interactions remain the same.
It is also not clear how they can incorporate prior knowledge on label structures.

The third group models label dependencies using graphical model representations~\cite{lafferty2001conditional,chen2019multi}.
%Recent attempts to use a label graph to model label correlation alleviate the two issues above and exhibit scalable performance.
%\citet{chen2019multi} use stacked graph convolution networks to learn label representations and map them into a set of inter-dependent object classifiers.
%However, with this method the results are not interpretable.
Methods within this group often build a label graph, in which a node corresponds to a label, and edges represent how two labels interact with each other.
Most recently, \citet{lanchantin2019neural} propose LaMP, where they apply the attention mechanism from Transformer~\cite{vaswani2017attention} to learn how other labels contribute to the presence/absence of a label.
Further, they use an MPNN, a generalization of graph neural networks (GNN)~\cite{scarselli2008graph}, to pass messages among label nodes weighted by attention, thus modelling a conditional joint representation of output labels.
%LaMP is most closely-related to this work: it provides a framework to reason about the correlation between labels using attention, and we extend it to model the joint representation of more labels, which is higher-order correlation learning.
Compared to PCC methods, LaMP provides a scalable and flexible module to model label correlations that requires no label ordering and allows parallel computation, and its graphical structure making it a natural fit to impose constraints on labels.
However, LaMP follows a encoder-to-decoder architecture, and learning feature embeddings within this architecture has not yet been optimized.
It does not incorporate any label information in the feature embedding, which has been shown to be beneficial for making accurate predictions~\cite{yeh2017learning}.

This work leverages both the state-of-the-art latent embedding learning and powerful attention-based MPNNs to provide an accurate and scalable multi-label classifier, and we further extend the message passing module to model high-order label correlations to improve performance.
%\SK{The lamp model you employed is actually the transformer used in NLP. Specially, it is a GPT-3. Try to carefully think about the connections to NLP and GNN here.}


%Though LaMP has a promising way of model label correlation, it remains unexplored what would be an effective way to build a feature-encoder-decoder branch and a label-encoder-decoder branch on top of MPNNs, which could help with learning better features.
%For what is particularly challenging, the feature branch and the label branch may output different sizes of embeddings; it then becomes unclear how to align two probabilistic latent spaces in a useful way.
%This work takes the first step to incorporate a complex message passing scheme into two-branch VAE-based encoder-decoder structure.

